Category-Level Multi-Part Multi-Joint 3D Shape Assembly

Shape assembly composes complex shapes geometries by arranging simple part geometries and has wide applications in autonomous robotic assembly and CAD modeling. Existing works focus on geometry reasoning and neglect the actual physical assembly process of matching and fitting joints, which are the contact surfaces connecting different parts. In this paper, we consider contacting joints for the task of multi-part assembly. A successful joint-optimized assembly needs to satisfy the bilateral objectives of shape structure and joint alignment. We propose a hierarchical graph learning approach composed of two levels of graph representation learning. The part graph takes part geometries as input to build the desired shape structure. The joint-level graph uses part joints information and focuses on matching and aligning joints. The two kinds of information are combined to achieve the bilateral objectives. Extensive experiments demonstrate that our method outperforms previous methods, achieving better shape structure and higher joint alignment accuracy.

==> 8_checklist.tex <==
\section{Check List}


\textbf{Reproducibility} For reproducibility of the empirical results we provided in the paper, we will open-source our training/inference code, dataset, and network weights. % Can you also release the Dataset?


\textbf{Responsible Machine Learning Research}
Our task and method aim to help autonomous systems to assemble furnitures and does not invade human rights and privacy. We are


\textbf{Research Ethics} Our research is original and conducted with synthetically generated data and only involves running experiments on computing resources.

\textbf{Transparency}
We will release all data and code associated with the paper experiments.

\textbf{Societal Impact}
Our work can positively benefit the robotics industries in the area of autonomous 3D shape assembly. The ability to partially automate the construction of 3D models with tailored parts has the potential to reduce costs and timelines by lessening tedious work. The success of this line of research is beneficial for furniture auto-assembly and 3D model design. 

Other negative impacts of our research on society are harder to predict, but it suffers from the same issues as most deep learning algorithms. These include privacy concerns and lack of interpretability, as well as other negative effects of increased automation. 

==> Tables_Alg/exp_baselines.tex <==
% 	\hspace{-5mm}
	\begin{table*}[t]
% 	\footnotesize{
        % \small 
     \resizebox{\textwidth}{!}{%
        \scriptsize
		\begin{center}
			\begin{tabular}{c|ccc|ccc|ccc|ccc}
				\toprule
				& \multicolumn{3}{c}{Shape Chamfer Distance $\downarrow$} & \multicolumn{3}{c}{Part Accuracy $\uparrow$} & \multicolumn{3}{c}{Joint Chamfer Distance $\downarrow$} & \multicolumn{3}{c}{Joint Accuracy $\uparrow$} \\ 
				\midrule
				% \hline
				% \hline % \midrule 
				& Chair & Table & Cabinet & Chair & Table & Cabinet & Chair & Table & Cabinet & Chair & Table & Cabinet \\
				  \midrule				% \hline
				B-Global& 0.015 & 0.013 & 0.008 & 32.8 & 30.1 & 33.6 & 0.712 & 0.847 & 0.667 & 13.4 & 15.8 & 10.7  \\
				% \hline % \midrule				
				B-LSTM & 0.017 & 0.026 & 0.007 & 39.4 & 22.5 & 44.4 & 0.756 & 0.728 & 0.651 & 17.0 & 13.2 & 14.8  \\
				% \hline %\midrule				
				B-Complement & 0.028 & 0.034 & 0.222 & 11.0 & 5.33 & 0.0 & 0.901 & 0.977 & 1.074 & 7.54 & 8.30 & 23.6  \\
				% \hline %\midrule				
				B-Dynamic  & 0.007 & 0.008 & 0.006 & 65.3 & 61.4 & 45.0 & 0.725 & 0.855 & 0.683 & 24.4 & 30.0 & 18.6    \\
			
				% \hline %\midrule	
				\textbf{Ours} & \textbf{0.006} & \textbf{0.007} &\textbf{ 0.005} & \textbf{72.8} & \textbf{67.4} & \textbf{63.3} & \textbf{0.352} & \textbf{0.602} & \textbf{0.620} & \textbf{57.2} & \textbf{50.6} & \textbf{27.5}  \\
				\bottomrule
			\end{tabular}
	    
		\end{center}
	} % resizebox
		\caption{Quantitative comparison between our approach and the baseline methods.}
		\label{table:performance}
% 		}
% 		\vspace{-0.2cm}
	\end{table*}	

==> Tables_Alg/table_ablation.tex <==
\begin{table}[!htb]
    
    \begin{minipage}[l]{.48\linewidth}
    %   \begin{flushleft}
      \centering
            \resizebox{\textwidth}{!}{%
                \begin{tabular}{c|c|c|c|c}
    				\toprule
    				& SCD $\downarrow$ & Part Acc. $\uparrow$ & JCD $\downarrow$ & Joint Acc. $\uparrow$ \\ 
    				% \hline
    				% \hline % \midrule 
    				% & Chair & Table & Cabinet & Chair & Table & Cabinet & Chair & Table & Cabinet & Chair & Table & Cabinet \\
    				  \midrule				% \hline
    				B-Global&  0.029 & 5.4 & 0.513 & 12.7   \\
    				% \hline % \midrule				
    				B-LSTM & 0.037 & 4.4 & 0.394 & 20.3  \\
    				% \hline %\midrule				
    				B-Complement &  0.048& 4.5 & 0.456 & 17.2 \\
    				% \hline %\midrule	0.034 & 11.5 & 0.379 & 21.5			
    				B-Dynamic  & 0.034 & 11.5 & 0.379 & 21.5   \\
    		
    				% \hline %\midrule	
    				% \textbf{Ours} & \textbf{	0.006} & \textbf{72.8 }& \textbf{0.352 }& \textbf{57.2} \\
    				\bottomrule
    			\end{tabular}
			} % resizebox
% 		\end{flushleft}
    \end{minipage}%
    \begin{minipage}[r]{.52\linewidth}
    % \begin{flushright}
      \centering
            \resizebox{\textwidth}{!}{%
                \begin{tabular}{c|c|c|c|c}
    				\toprule
    				& SCD $\downarrow$ & Part Acc. $\uparrow$ & JCD $\downarrow$ & Joint Acc. $\uparrow$ \\ 
    				% \hline
    				% \hline % \midrule 
    				% & Chair & Table & Cabinet & Chair & Table & Cabinet & Chair & Table & Cabinet & Chair & Table & Cabinet \\
    				  \midrule				% \hline
    				w/o matching alg.& 0.010 & 55.1 & 0.416 & 37.5  \\
    				% \hline % \midrule				
    				w/o rotation operator & 0.009 & 58.2 & 0.350 & 46.1 \\
    				% \hline %\midrule				
    				w/o joint embedding & 0.019 & 33.4 & 0.258 & 36.9 \\
    				% \hline %\midrule				
    				Ours full & 0.006 & 72.8 & 0.352 & 57.2     \\
    			
    				% \hline %\midrule	
    				% \textbf{Ours} & \textbf{0.006} & \textbf{0.007} &\textbf{ 0.005} & \textbf{72.8}  \\
    				\bottomrule
    			\end{tabular}
			} % resizebox
% 	\end{flushright}
    \end{minipage} 
    \caption{Left: Right:}
\end{table}

==> notes.tex <==
Data generated by networks of mobile and IoT devices poses unique challenges for training machine learning models. Due to the growing storage/computational power of these devices and concerns about data privacy, it is increasingly attractive to keep data and computation locally on the device~\cite{federated_mtl}. 
\textit{Federated Learning (FL)} ~\cite{mohassel2018aby,federated_secure,secureml} provides a privacy-preserving mechanism to effectively leverage such decentralized data and computation resources to train machine learning models. The main idea behind FL is to have each node learn on its own local data and only send gradient updates to the central server, which updates the global model. 

While federated learning promises better privacy and efficiency, existing methods ignore the fact that the data on each node are collected in a non-\textit{i.i.d} manner, leading to \textit{domain shift}~\cite{datashift_book2009} between nodes. For example, one device may take photos mostly indoors, while another mostly outdoors. In this paper, we address the problem of transferring knowledge from the decentralized nodes to a new node with a different data domain, without requiring any additional supervision from the user. We call this problem \textit{Unsupervised Federated Domain Adaptation} (UFDA).

There is a large body of existing work on unsupervised domain adaptation (e.g.,~\cite{long2015,DANN,adda,CycleGAN2017, gong2012geodesic, long2018conditional}), but the federated setting presents several additional challenges. First, the data are stored locally and cannot be shared, which hampers mainstream domain adaptation methods as they need to access both the labeled source and unlabeled target data~\cite{ddc, JAN, ghifary2016deep, SunS16a, DANN, adda}. Second, the model parameters are trained separately for each node and converge at different speeds, while also offering different contributions to the target node depending on how close the two domains are. Finally, the knowledge learned from source nodes is highly entangled~\cite{bengio2013representation}, which can lead to \textit{negative transfer}~\cite{pan2010survey}.

In this paper, we propose a solution to the above problems called \textit{Federated Adversarial Domain Adaptation} (FADA) which aims to tackle domain shift in a federated learning system through adversarial techniques.
Our approach preserves data privacy by training one model per source node  and updating the target model with the aggregation of source gradients, but does so in a way that reduces domain shift.  
First, we analyze the federated domain adaptation problem from a theoretical perspective and provide a generalization bound. Inspired by our theoretical results, we propose an efficient adaptation algorithm based on adversarial adaptation techniques applied to the federated setting. We also devise a \textit{dynamic attention} model to cope with the varying convergence rates in the federated learning system.
We conduct extensive experiments on real-world datasets, including both image classification and natural language tasks. Compared to baseline methods, we improve adaptation performance on all tasks, demonstrating the effectiveness of our model.

==> tmp.tex <==
Compared to the centralized training approach, federated learning is a decentralized training approach which enables mobile phones located at different geographical locations to collaboratively learn a machine learning model while keeping all the personal data that may contain private information on device.

Federated learning provides a privacy-preserving mechanism to effectively leverage those decentralized compute resources inside end devices to train machine learning models.
